Distance Encoding: Design Provably More Powerful Neural Networks for Graph Representation Learning

Learning representations of sets of nodes in a graph is crucial for applications ranging from node-role discovery to link prediction and molecule classification. Graph Neural Networks (GNNs) have achieved great success in graph representation learning. However, expressive power of GNNs is limited by the 1-Weisfeiler-Lehman (WL) test and thus GNNs generate identical representations for graph substructures that may in fact be very different. More powerful GNNs, proposed recently by mimicking higher-order-WL tests, only focus on representing entire graphs and they are computationally inefficient as they cannot utilize sparsity of the underlying graph. Here we propose and mathematically analyze a general class of structure-related features, termed Distance Encoding (DE). DE assists GNNs in representing any set of nodes, while providing strictly more expressive power than the 1-WL test. DE captures the distance between the node set whose representation is to be learned and each node in the graph. To capture the distance DE can apply various graph-distance measures such as shortest path distance or generalized PageRank scores. We propose two ways for GNNs to use DEs (1) as extra node features, and (2) as controllers of message aggregation in GNNs. Both approaches can utilize the sparse structure of the underlying graph, which leads to computational efficiency and scalability. We also prove that DE can distinguish node sets embedded in almost all regular graphs where traditional GNNs always fail. We evaluate DE on three tasks over six real networks: structural role prediction, link prediction, and triangle prediction. Results show that our models outperform GNNs without DE by up-to 15\% in accuracy and AUROC. Furthermore, our models also significantly outperform other state-of-the-art methods especially designed for the above tasks.

==> 06_broaderimpact.tex <==
\section*{Broader Impact}
This work proposes a novel angle to systematically improve the structural representation power of GNNs. We break from the convention that previous works characterize and further improve the power of GNNs by intimating different-order WL tests~\cite{chen2019equivalence,maron2019provably,morris2019weisfeiler,chen2020can}. As far as we know, we are the first one to provide non-asymptotic analysis of the power of the proposed GNN models. Therefore, the proof techniques of Theorems~\ref{thm:power},\ref{thm:limit} may be expected to inspire new theoretical studies of GNNs and further better the practical usage of GNNs. Moreover, our models have good scalability by avoiding using the framework of WL tests, as higher-order WL tests are not able to leverage the sparsity of graphs. To be evaluated over extremely large graphs~\cite{hu2020open}, our models can be simply trimmed and work on the ego-networks sampled with a limited size around the target node sets, just as the strategy adopted by GraphSAGE~\cite{hamilton2017inductive} and GraphSAINT~\cite{zeng2019graphsaint}. \textbf{Therefore, our work may  motivate practitioners to design and deploy more powerful GNNs in industrial pipelines to benefit the society.}

Distance encoding unifies the techniques of many GNN models~\cite{zhang2018link,abu2019mixhop,chen2019path,maziarka2020molecule,klicpera2019diffusion} and provides a extremely general framework with clear theoretical characterization. In this paper, we only evaluate four specific instantiations over three levels of tasks. However, there are some other interesting instantiations and applications. For example, we expect a better usage of PageRank scores as edge attributes (Eq.~\eqref{eq:agg-pe}). Currently, our instantiation DEAGNN-PR simply uses those scores as weights in a weighted sum to aggregate node representations. We also have not considered any attention-based mechanism over DEs in aggregation while it seems to be useful~\cite{velivckovic2017graph,maziarka2020molecule}. Researchers may try these directions in a more principled manner based on this work. Our approaches may also help other tasks based on structural representation learning, such as graph-level classification/regression~\cite{gilmer2017neural,zhang2018end,xu2018powerful,maron2019provably,morris2019weisfeiler} and subgraph counting~\cite{chen2020can}, which correspond to \textbf{many applications with wide societal impact including drug discovery and structured data analysis.} %As this paper has already covered broad content, the evaluation over these new applications are left out and may inspire researchers and practitioners for further investigation. 

There are also two important implications coming from the observations of this work. First, Theorem~\ref{thm:limit} and Corollary~\ref{col:PEAGNN} show the limitation of DE-1 over distance regular graphs, including the cases when DE-1's are used as node attributes or controllers of message aggregation. As distance regular graphs with the same intersection array have the important co-spectral property~\cite{brouwer2012distance}, we guess that DE-1 is a bridge  to connect GNN frameworks to spectral approaches, two fundamental approaches in graph-structured data processing. This point sheds some light on the question left in \cite{chen2019equivalence} while more rigorous characterization is still needed. Second, as observed in the experiments, higher-order DE's induce larger gains as opposed to WLGNN, while Theorem~\ref{thm:power} is not able to characterize this observation as the probability $1-o(\frac{1}{n})$ does not depend on the size $p$. We are sure that the probabilistic quantization in Theorem~\ref{thm:power} is not tight, so it is interesting to see how such probability depends on $p$ by deriving tighter bounds.

\textbf{We are not aware of any societal disadvantages of this research. Our experiments also do not leverage biases in the data.} We choose those datasets based on two rules that are irrelavant to ethics: (1) The labels for evaluation are graph-structured related; (2) Those datasets were used in some baselines so that we provide fair comparison. Regarding the point (1), this is the reason that we do not use the datasets, such as Cora, Citeseer and Pubmed~\cite{sen2008collective}, whose node labels that indicate the community belongings of nodes instead of the structural function of nodes. However, it is interesting to evaluate distance encoding techniques over those datasets with community-related labels in the future. %People who want to use our approach over other datasets should be careful about whether there is some underlying bias introduced by distance encoding. 


\section*{Acknowledgements}
The authors would like to thank Weihua Hu for raising the preliminary concept of distance encoding that initializes the investigation. The authors also would like to thank Jiaxuan You and Rex Ying for their insightful comments during the discussion. The authors also would thank Baharan Mirzasoleiman and Tailin Wu for their suggestions on the paper writing. The authors also would like to thank the NeurIPS reviewers for their insightful observations and actionable suggestions to improve the manuscript. This research has been supported in part by Purdue CS start-up, NSF CINES, NSF HDR, NSF Expeditions, NSF RAPID, DARPA MCS, DARPA ASED, ARO MURI, Stanford Data Science Initiative, Wu Tsai Neurosciences Institute, Chan Zuckerberg Biohub, Amazon, Boeing, Chase, Docomo, Hitachi, Huawei, JD.com, NVIDIA, Dell. J. L. is a Chan Zuckerberg Biohub investigator.
